Deterministic and game separability for regular languages of infinite trees

We show that it is decidable whether two regular languages of infinite trees are separable by a deterministic language, resp., a game language. We consider two variants of separability, depending on whether the set of priorities of the separator is fixed, or not. In each case, we show that separability can be decided in EXPTIME, and that separating automata of exponential size suffice. We obtain our results by reducing to infinite duration games with {\omega}-regular winning conditions and applying the finite-memory determinacy theorem of B\"uchi and Landweber.

==> 5_gam_gen_new.tex <==
\section{Separability by game automata}
\label{sec:gam_gen}

Fix two automata $\A$ and $\B$. Without loss of generality assume that the sets of states of these automata are disjoint. Consider the following positionless game\=/separability game $\GameSeparabilityGame \A \B$.

\begin{gamebox}{Game\=/separability game $\GameSeparabilityGame \A \B$}
    \begin{enumerate}
        \item \Input plays a letter $a_i \in \Sigma$.
        \item \Separator plays a splitter\footnote{If $f_i \in \set{\L, \R}^{\Delta^\A(a_i)}$ then we say that it is an~$\A$\=/splitter, and if $f_i \in \set{\L, \R}^{\Delta^\B(a_i)}$ then $f_i$ is a~$\B$\=/splitter.} $f_i \in \set{\L, \R}^{\Delta^\A(a_i)}\cup \set{\L, \R}^{\Delta^\B(a_i)}$
        \item \Input plays a direction $d_i \in \set{\L, \R}$.
    \end{enumerate}
\end{gamebox}

Let the resulting infinite play be $\pi = \tuple{a_0, f_0, d_0} \tuple{a_1, f_1, d_1} \cdots$,
with the induced infinite branch $b := \tuple{a_0, d_0} \tuple{a_1, d_1} \cdots$.

\Separator wins the play $\pi$
if at least one of the two conditions below fail:
%
\begin{itemize}
\item $\Win_\A(\pi)$:~There is an~accepting sequence of transitions
    $\vec\delta^\A = \delta_0^\A \delta_1^\A \cdots \in \Delta^\A(b)$
	such that for every $i\in\omega$ if $f_i$ is an~$\A$\=/splitter then $f_i(\delta_i^\A) = d_i$.
\item $\Win_\B(\pi)$:~There exists an accepting sequence of transitions
    $\vec\delta^\B = \delta_0^\B \delta_1^\B \cdots \in \Delta^\B(b)$
	such that for every $i\in\omega$ if $f_i$ is a~$\B$\=/splitter then $f_i(\delta_i^\B) = d_i$.
\end{itemize}

\begin{lemma}
    \label{lem:game:sep}
    \Separator wins the separability game $\GameSeparabilityGame \A \B$
    if, and only if, there exists a game automaton $\S$ separating $\lang \A$ from $\lang \B$.
\end{lemma}

\subparagraph*{Soundness}

Assume that \Separator wins the separability game $\GameSeparabilityGame \A \B$ by a~finite\=/memory winning strategy $\M = \langle M, \ell_0, \overline{f}, \tau\rangle$ which has one decision function $\overline{f}$ which assigns to each $\ell\in M$ and $a\in\Sigma$ a~splitter $\overline{f}(\ell,a)\in\set{\L, \R}^{\Delta^\A(a)}\cup\set{\L, \R}^{\Delta^\B(a)}$. Moreover, the type of the memory update function is $\tau\colon M\times\Sigma\times \set{\L, \R}\to M$.

Consider a~game automaton
$\S := \langle \Sigma, M\cup\{\top\}, \ell_0, \Omega^\S, \Delta^\S\rangle$
which has the same set of states $M$ (plus the additional state $\top$) and initial state $\ell_0$ as $\M$,
priorities are induced by the decision function $\overline{c}$ of $\M$ as
$\Omega^\S(\ell) := \overline{c}(\ell)$, $\Omega^\S(\top)=0$, and
and transitions for $q\in M$ and $a\in\Sigma$ are of the form
\[
\Delta^\S(q,a) = 
	\begin{cases}
		\set{\tuple{\ell,a,\ell_\L, \top}, \tuple{\ell,a,\top,\ell_\R}}
        &\text{if $\overline{f}(\ell, a)$ is an~$\A$\=/splitter,}\\
        \set{\tuple{\ell,a,\ell_\L, \ell_\R}}
        &\text{if $\overline{f}(\ell, a)$ is a~$\B$\=/splitter,}\\
	\end{cases}
\]   
where $\ell_\L := \tau(\ell, a, \L)$ and $\ell_\R := \tau(\ell, a, \R)$. We show that $\S$ separates $\lang \A$, $\lang \B$.

=======================================

\begin{proof}
    We prove the two directions separately.

    \subparagraph{``Only if'' direction.}

    For the ``only if'' direction, assume that \Separator wins the game separability game
    %
    \begin{align*}
        G_0 := \GameSeparabilityGame \A \B,
    \end{align*}
    %
    and we show that there exists a game automaton $\S$ separating $\lang \A$ from $\lang \B$.
    %
    Since the winning condition of the separability game is $\omega$\=/regular,
    by \cref{thm:BuchiLandweber} there exists a~finite\=/memory winning strategy
    $\M = \langle M, \ell_0, \overline{f}, \tau\rangle$.
    %
    %
    We build a separating game automaton $\S := \langle \Sigma, M\sqcup\{\top\}, \ell_0, \Delta^\S, W\rangle $
    where $\Sigma$ is the input alphabet,
    the set of states is $M$,
    the generalised acceptance condition $W$ will be discussed below,
    and transitions in $\Delta^\S$ are of the form
    %
	\[
        \Delta^\S(\ell, a) =
			\begin{cases}
			    \set{\tuple{\ell,a,\ell_\L, \top}, \tuple{\ell,a,\top,\ell_\R}}
                & \text{if $\overline{m}(\ell, a) = \lor $,}\\
            	\set{\tuple{\ell,a,\ell_\L, \ell_\R}}
                & \text{if $\overline{m}(\ell, a) = \land$,}
			\end{cases}
    \]    
    where $\ell_\L := \tau(\ell, a, \L)$ and $\ell_\R := \tau(\ell, a, \R)$.
    
\michal{We invoke the acceptance game below\ldots}

    The generalised acceptance condition $W$ of the automaton $\S$ is defined as follows.
    Consider an~infinite play of $\S$'s acceptance game $\AcceptanceGame \S t$
    of the form $\pi' = \tuple{\ell_0,a_0,d_0}\tuple{\ell_1,a_1,d_1} \cdots$.
    Let $\vec f = f_0f_1\cdots$ be the infinite sequence of decision functions where, for every $i$,
    $f_i=\overline{f}(\ell_i, a_i)$.
    % Consider an infinite branch $b = a_0d_0 a_1d_1 \cdots$,
    % and let $f_0f_1 \cdots$ be the corresponding sequence of choice functions as determined by \Separator.
    % %
    % (Formally, this is defined with the help of the auxiliary sequence of memory locations $\ell_0 \ell_1 \cdots$
    % by induction as:
    % $\ell_0$ is the initial memory location of $\M$,
    % $f_n$ is the second component of $\delta_\M(\ell_n, a_n) = \tuple{\_, f_n}$,
    % and $\ell_{n+1} = \delta_\M(\tuple{\ell_n, a_n}, d_n)$.)
    %
\michal{For the sake of consistency, I'd use $W\A(\pi)$ and $W\B(\pi)$. Also in other places we can change W1 and W2 into $W\A$ and $W\B$, no?}

    Let $\phi_\A'(\pi')$ hold if, and only if, $\phi_\A(\pi)$ holds,
    where $\pi = \tuple {a_0,f_0,d_0} \tuple{a_1,f_1,d_1} \cdots$ is the infinite play of the separability game $\GameSeparabilityGame \A \B$
    obtained from $\pi'$ and the sequence of choice functions $\vec f$ induced by Separator's strategy $\M$.
    %
    Similarly, let $\phi_\B'(\pi')$ hold if, and only if, $\phi_\B(\pi)$ holds.
    %
    The two predicates $\phi_\A'$, $\phi_\B'$ depend on \Separator's winning strategy $\M$, which we have already fixed.
    Since $\M$ is winning, $\phi_\A$, $\phi_\B$ are disjoint (as languages of plays of the separability game $G_0$),
    and consequently so are $\phi_\A'$, $\phi_\B'$ (as languages of plays of the acceptance game for $\S$).
\michal{this disjointness is also once restricted to the plays consistent with his strategy\ldots}
    %
    Take as the generalised acceptance condition of $\S$ any regular language $W$ separating $\phi_\A'$, $\phi_\B'$,
    i.e., s.t.~$\phi_\A' \subseteq W \disjoint \phi_\B'$.
    %
    (The simplest such option can be $W := \phi_\A'$ itself.)
    
    \lorenzo{We use the acceptance game below.}

    We show that $\S$ separates $\lang \A$ from $\lang \B$.
    In order to show $\lang \A \subseteq \lang \S$, let $t \in \lang \A$.
    Thus \Automaton wins the acceptance game $G_1 := \AcceptanceGame \A t$ against \Pathfinder.
    %
    We show that \Automaton likewise wins the acceptance game $G_2 := \AcceptanceGame \S t$.
    %
    To show this we play in parallel the separability game $G_0$ and the two acceptance games $G_1$ and $G_2$.
    %
    As we play all games in locksteps, we maintain the following invariant:
    At every round $i$,
    the current finite branch of the input tree $t$ is $b_i = \tuple{a_0,d_0} \cdots \tuple{a_{i-1}, d_{i-1}}$,
    \Separator's winning strategy $\M$ in the separability game $G_0$ is in memory state $\ell_i$,
    this is also the current state of the separating automaton $\S$ in the acceptance game $G_2$,
    and the current state of $\A$ in the acceptance game $G_1$ is $p_i$.
    %
    Let now be at round $i$ and assume that the invariant holds.
    %
    The next input symbol to be read in the acceptance games $G_1$ and $G_2$ is $a_i := t(d_0 \cdots d_{i-1})$.
    %
    We let \Input play $a_i$ in the separability game $G_0$.
    We also let \Automaton choose a transition
    %
    \begin{align*}
        \delta^\A_i = (p_i, a_i, p_{\L,i}, p_{\R,i})
    \end{align*}
    %
    in the acceptance game $G_1$.
    Let \Separator respond with a choice function $f_i$ according to her winning strategy $\M$:
    %
    \begin{align*}
        \overline{f}(\ell_i, a_i) = f_i.
    \end{align*}
    %
    We distinguish two cases.
    %
    \begin{enumerate}

        \item In the first case, assume \Separator played $\overline{m}(\ell,a_i)=\lor$ and $f_i \in \set{\L, \R}^{\Delta^\A(a_i)}$.
        %
        Thus it is \Automaton's responsibility to choose a direction in the acceptance game $G_2$,
        and to this end we let her choose $d_i := f_i(\delta^\A_i)$,
        conforming to \Separator's winning strategy.        

        \item In the second case, \Separator played a conjunctive choice function
        %
        \begin{align*}
            f_i = f_i^\land \in \set{\L, \R}^{\Delta^\B(a_i)},
        \end{align*}
        %
        Thus it is \Pathfinder's duty to choose a direction $d_i$ in the acceptance game $G_2$,
        and thus we consider an arbitrary such $d_i$.

    \end{enumerate}
    %
    In either of the two cases above, we now have a new direction $d_i$,
    which is used to update the acceptance game $G_1$ by letting \Pathfinder play it.
    %
    Thus the new state of $\A$ in $G_1$ is $p_{i+1} := p_{d_i,i}$
    (i.e., $p_{\L,i}$ or $p_{\R,i}$ according to the chosen direction $d_i$),
    the new state of $\S$ in $G_2$ and the new memory location of $\M$ in $G_0$ is
    %
    \begin{align*}
        \ell_{i+1} := \tau(\ell_i, a_i, d_i).
    \end{align*}
    %
    This concludes the description of round $i$ of all three games.
    We argue that \Automaton wins the resulting infinite play of the acceptance game $G_2$.
    Consider the infinite play $\pi = \tuple{a_0, f_0, d_0} \tuple{a_1, f_1, d_1} \cdots$ of the separability game $G_0$.
    %
    Since \Automaton wins in $G_1$, the infinite sequence of $\A$'s transitions $\delta_0^\A \delta_1^\A \cdots$ is accepting.
    By definition, whenever $f_i = f^\lor$ we have $f^\lor(\delta_i^\A) = d_i$.
    It follows that $\pi\in\phi_\A$ holds.
    %
    By definition, $\pi' \in \phi_\A'$ holds on the corresponding infinite play
    $\pi' = \tuple{\ell_0, a_0, d_0} \tuple{\ell_1,a_1, d_1} \cdots$ of $G_2$.
\michal{above we have memory states $\ell_i$ in the play :(}
    %
    Since $\S$'s generalised acceptance condition $W$ by definition satisfies $\phi_\A' \subseteq W$,
    we have that $\pi' \in W$ is accepting
    and thus \Automaton wins the infinite play in $G_2$, as required.
    %
    This concludes the argument establishing $\lang \A \subseteq \lang \S$.

    We now need to show that $\lang \S \disjoint \lang \B$,
    which is the same as $\lang \B \subseteq \lang {\S^\mathrm c}$,
    where the dual game automaton $\S^\mathrm c$ recognises the complement language of $\S$.
\michal{We should define the ``dual game automaton''}
    %
    Since $W \disjoint \phi_\B'$ by definition of $W$,
    we have $\phi_\B' \subseteq W^\mathrm c$.
    %
    We can thus conclude by applying the same argument as in the first part above
    with $\A$ replaced by $\B$,
    and $\S$ replaced by $\S^\mathrm c$.

    \subparagraph*{``If'' direction.}

    For the ``if'' direction, assume that the game automaton $\S$ separates $\lang \A$ from $\lang \B$
    and we show that \Separator wins the separability game.
    %
    By slightly rephrasing the separation condition,
    we have $\lang \A \bot \lang {\S^\mathrm c}$ and $\lang \B \bot \lang \S$,
    where $\S^\mathrm c$ is $\S$'s dual game automaton recognising the complement of $\lang \S$.
    
    Since the two languages $\lang \B$ and $\lang \S$ are disjoint,
    \Pathfinder wins the disjointness game $G_2 := \DisjointnessGame \B \S$.
    %
\michal{below we have ``positions'', at the moment there is no such thing in our games, but I'm afraid that we'll need them :(}
    By unravelling the definition of the product automaton $\B \times \S$,
    we have that a position in $G_2$ is a pair of the form $\tuple{p^\B, p^\S}$
    where $p^\B$ is a state of $\B$ and $p^\S$ is a state of $\S$.
    %
    By the definition, \Pathfinder wins an infinite play
    $\pi_2 = \tuple{\tuple{p^\B_0, p^\S_0}, a_0, d_0} \tuple{\tuple{p^\B_1, p^\S_1}, a_1, d_1}\cdots$ of $G_2$
    whenever either the first projection $\pi_2^\B = \tuple{p^\B_0, a_0, d_0} \tuple{p^\B_1, a_1, d_1}\cdots$ is rejecting in $\B$
    (i.e., $\Omega^\B(\pi_2^\B) = \Omega^\B(p^\B_0) \Omega^\B(p^\B_1) \cdots$ is rejecting),
    or the second projection $\pi_2^\S = \tuple{p^\S_0, a_0, d_0} \tuple{p^\S_1, a_1, d_1}\cdots \not\in W^\S$ is rejecting in $\S$
    (i.e., $\Omega^\S(\pi_2^\S) = \Omega^\S(p^\S_0) \Omega^\S(p^\S_1) \cdots$ is rejecting).
    %
    Since the acceptance conditions of both $\B$ and $\S$ are parity conditions,
    so are their complements.
    %x
    Since parity conditions are Rabin conditions
    and the latter are closed under disjunction,
    we have that \Pathfinder's winning condition in $G_2$ is a Rabin condition.
    %
\michal{This fact should appear in the preliminaries}
    Since games with Rabin winning conditions are memoryless determined \cite[Lemma 9]{Klarlund:APAL:1994}
    (c.f.~also \cite[Theorem 4]{Graedel:STACS:2004} and \cite[Theorem 7.12]{Kopczynski:PhD:2008}),
    it follows that \Pathfinder has a memoryless winning strategy in $G_2$.
    %
    From now on we fix a memoryless winning strategy for \Pathfinder in $G_2$
    and the same for the disjointness game $G_1 := \DisjointnessGame \A {\S^\mathrm c}$.

    We maintain the invariant that at round $i$ of the separability game
    the separating automaton $\S$ is in state $p_i^\S$.
    % the nonemptiness game $G_1$ is in position $\tuple {p_i^\A, p_i^\S}$
    % and the nonemptiness game $G_2$ in $\tuple{p_i^\B, p_i^\S}$
    % (thus the separating automaton is in the same state $p_i^\S$ in both games).
    %
    Let \Input play a letter $a_i \in \Sigma$ in the separability game $G_0$.
    Let $\Delta^\A(a_i)$ be the set of all transitions in $\A$ over $a_i$,
    and similarly for $\Delta^\B(a_i)$.
    %
    There are two cases to consider.
    %
    \begin{enumerate}

        \item In the first case,
        $\delta(p_i^\S, a_i) = \tuple{p^\S_\L, \L} \land \tuple{p^\S_\R, \R}$ is a conjunctive transition.
        We look at the nonemptiness game $G_2 = \Game {\B \times \S}$ and at \Pathfinder's memoryless winning strategy therein.
        %
        \Separator plays in $G_0$ the conjunctive choice function $f_i^\land \in \set {\L, \R}^{\Delta^\B(a_i)}$ defined as follows.
        On input $\delta^\B = \tuple{p^\B, a_i, p^\B_\L, p^\B_\R} \in \Delta^\B$,
%        if $a \neq a_i$, then $f_i^\land(\delta^\B)$ is defined arbitrarily (e.g., $f_i^\land(\delta^\B) := \L$).
%        If $a = a_i$, then
        consider position $\tuple {p^\B, p_i^\S}$ of $G_2$
        and let \Automaton play $a_i \in \Sigma$
        and transitions $\delta^\B$, $\delta^\S = \tuple{p_i^\S, a_i, p_\L, p_\R}$.
        %
        \Pathfinder applies her memoryless winning strategy to obtain a direction $d \in \set {\L, \R}$.
        We then define $f_i^\land(\delta^\B) = d$.

        \item In the second case,
        $\delta(p_i^\S, a_i) = \tuple{p^\S_\L, \L} \lor \tuple{p^\S_\R, \R}$ is a disjunctive transition,
        and thus it is a conjunctive transition $\delta(p_i^{\S^\mathrm c}, a_i) = \tuple{p^{\S^\mathrm c}_\L, \L} \land \tuple{p^{\S^\mathrm c}_\R, \R}$
        in the complement automaton $\S^\mathrm c$.
\michal{sets of transitions, not Boolean formulae above}
        %
        We now look at the disjointness game $G_1 = \DisjointnessGame \A {\S^\mathrm c}$
        and, by applying \Pathfinder's winning strategy therein in an analogous manner as in the previous point,
        we obtain a disjunctive choice function $f_i^\lor \in \set {\L, \R}^{\Delta^\A(a_i)}$.
        \Separator then plays $f_i^\lor$ in $G_0$.
        
    \end{enumerate}
    %
    We now let \Input play a direction $d_i \in \set{\L, \R}$
    and define $p_{i+1}^\S = p^\S_{d_i,i}$ in preparation for the next round.

    We now argue that \Separator wins the corresponding infinite play
    $\pi = \tuple{a_0,f_0,d_0} \tuple{a_1,f_1,d_1} \cdots$.
    %
    Let $b = \tuple{a_0,d_0}\tuple{a_1,d_1}\cdots$ be the corresponding branch.
    %
    By way of contradiction, assume that \Separator loses,
    i.e., both $\phi_\A(\pi)$ and $\phi_\B(\pi)$ hold.
    %
    Since $\phi_\B(\pi)$ holds,
    there exists an accepting sequence of transitions
    $\vec\delta^\B = \delta_0^\B\delta_1^\B\cdots \in \Delta^\B(b)$ in $\B$ over the branch $b$.
    
    This allows us to play the disjointness game $G_1 = \DisjointnessGame \B \S$ as follows.
    %
    We will maintain the following invariant:
    %
    At round $i$ the disjointness game $G_1$ is in configuration $\tuple{p_i^\B, p_i^\S}$
    and $\delta_i^\B = \tuple{p_i^\B, a_i, p_{\L,i}^\B, p_{\R,i}^\B} \in \Delta^\B(a_i)$
    is an $a_i$-transition of $\B$ from state $p_i^\B$.
    %
    Recall that \Pathfinder's strategy has been fixed at the beginning as a memoryless winning strategy.
    %
    We let \Automaton play round $i$ as follows.
    %
    She chooses input symbol $a_i$ and transition $\delta_i^\B$ in $\B$.
    The transition in $\S$ is determined as follows.
    %
    If $\delta^\S(p_i^\S, a_i) = \tuple{p_\L^\S, \L} \land \tuple{p_\R^\S, \R}$ is a conjunctive transition,
    then \Automaton chooses precisely this transition $\delta_i^\S := \tuple{p_i^\S, a_i, p_{\L,i}^\S, p_{\R,i}^\S}$
    (there is no other option in fact).
    %
    If $\delta^\S(p_i^\S, a_i) = \tuple{p_{\L,i}^\S, \L} \lor \tuple{p_{\R,i}^\S, \R}$ is a disjunctive transition
    %
    (which we represent as the set
    $\set{\delta_{\L,i}^\S, \delta_{\R,i}^\S}$,
    where $\delta_{\L,i}^\S := \tuple{p_i^\S, a_i, p^\S_{\L,i}, \top}$,
    and $\delta_{\R,i}^\S := \tuple{p_i^\S, a_i, \top, p^\S_{\R,i}}$),
    %
    then \Automaton uses the direction $d_i$ from $\pi$ and chooses transition 
    $\delta_{i, d_i}^\S$ accordingly.
    
    Round $i$ of the disjointness game $G_2$ is concluded with \Pathfinder playing a direction.
    %
    This direction must be $d_i$ for \Pathfinder to be winning (as we assumed),
    as we now argue.
    %
    On the one hand,
    if $\delta^\S(p_i^\S, a_i)$ is a conjunctive transition,
    then \Pathfinder by definition plays direction $f_i^\land(\delta_i^\B)$,
    and thanks to $\phi_\B(\pi)$, we have $f_i^\land(\delta_i^\B) = d_i$, as required.
    %
    On the other hand,
    if $\delta^\S(p_i^\S, a_i) = \tuple{p_{\L,i}^\S, \L} \lor \tuple{p_{\R,i}^\S, \R}$ is a disjunctive transition,
    then first \Automaton has played transition $\delta_{i, d_i}^\S$.
    %
    There are two cases to consider.
    If $d_i = \L$ and thus \Automaton has played $\delta_{i, \L}^\S := \tuple{p_i^\S, a_i, p^\S_{\L,i}, \top}$,
    then playing direction $\R$ would be losing for \Automaton
    since we assume that all states of $\B$ are productive,
    and thus there would exists some tree accepted from state $\tuple{p_{\R,i}^\B, \top}$ of the product automaton $\B \times \S$
    (where we regard $\top$ as a fictitious state recognising every tree).
    %
    This contradicts that \Pathfinder is playing according to a winning strategy in $G_2$;
    consequently, \Pathfinder must play $\L$ in this case.
    %
    The other case $d_i = \R$ is entirely symmetrical.
    %
    Thus, \Pathfinder chooses precisely direction $d_i$,
    and this ends the $i$-th round of $G_2$
    with the game going to configuration
    $\tuple{p_{i+1}^\B, p_{i+1}^\S} = \tuple{p_{d_i, i}^\B, p_{d_i, i}^\S}$,
    thus re-establishing the invariant as required.

    Let $\pi_2 = \tuple{\tuple{p^\B_0, p^\S_0}, a_0, d_0} \tuple{\tuple{p^\B_1, p^\S_1}, a_1, d_1}\cdots$
    be the resulting infinite play of the disjointness game $G_2$.
    %
    Since \Automaton plays as to ensure an accepting run
    $\pi_2^\B = \tuple{p^\B_0, a_0, d_0} \tuple{p^\B_1, a_1, d_1}\cdots$ in $\B$
    but \Pathfinder wins $G_2$,
    it must be the case that the second projection
    $\pi_2^\S = \tuple{p_0^\S, a_0, d_0} \tuple{p_1^\S, a_1, d_1} \cdots$ from the separating automaton $\S$ must be rejecting.

    Now we can repeat this whole argument for $\phi_\A(\pi)$ and the disjointness game $G_1 = \DisjointnessGame \A {\S^\mathrm c}$,
    deducing that the same sequence $\pi_2^\S = \tuple{p_0^\S, a_0, d_0} \tuple{p_1^\S, a_1, d_1} \cdots$
    from the complement separating automaton $\S^\mathrm c$ must be rejecting as well,
    i.e., it must be accepting as a sequence from $\S$, which is the sought contradiction.
\end{proof}

\begin{theorem}
    The game separability problem is decidable.
\end{theorem}

==> 8_conclus.tex <==

\section{Conclusions}
\label{sec:conclus}

\michal{I'd gladly see a short conclusions, even a single paragraph, not to finish with the last proof. You had some version of it, no?}

